RoamFlow: Reinforcement-Aligned One-Step Action MeanFlow Policy for Image-Goal Navigation

Image-goal navigation is a key challenge in embodied robotics, where an agent must reach a target specified solely by a goal image. While existing reinforcement learning approaches map perceptual observations directly to actions, they struggle to model long-horizon dependencies, often leading to suboptimal trajectories. To address this limitation, we propose RoamFlow, a generative navigation framework that leverages MeanFlow to predict the average velocity field for trajectory synthesis, enabling efficient few-step generation and reducing inference latency. We further adopt a two-stage training strategy that combines expert imitation for stable initialization with reinforcement learning for task-specific policy refinement. Extensive experiments in both Habitat simulation and real-world robotic platforms demonstrate that RoamFlow achieves efficient inference while maintaining strong navigation performance under real-time constraints.

==> zzx_experiment/4.Experiments.tex <==

\section{Experiments}

\subsection{Environmental Setup}%~\cite{puig2023habitat3}
In simulation, we use Habitat[] as our experimental platform and the training and evaluation pipeline. 

\subsubsection{Tasks setting}
We formulate navigation as a goal-conditioned policy learning problem.
Without relying on global localization, the agent navigates on a graph $M=\{V,E\}$, 
where nodes $V$ correspond to keyframes extracted from pre-collected expert trajectories, and edges $E$ denote traversable connections that encode topological constraints.To ensure feasibility under the topological prior, the agent is initialized at the starting pose of an expert trajectory. In each episode, given a distant goal image $I_g$, the agent performs self-localization on the topological map using the current RGB-D observation and plans a sequence of sub-goals (\textit{Sub-goals}). Finally, the policy outputs continuous velocity control commands to steer the agent toward the goal.


In the simulated environment, the agent is modeled as a planar differential-drive disc robot and is approximated by a circular collision proxy. 
We set the robot radius to $r = 0.1$ m and mount a forward-facing RGB-D camera with a $90^\circ$ horizontal field of view for perception. 
For control, each decision step is executed through continuous linear and angular velocity commands $(v_t, \omega_t)$, which are held for 1 s. 
To maintain high physical fidelity, these commands are applied via differential-drive kinematic integration at an execution rate of 10 Hz. During evaluation, an episode is considered successful when the agent issues the \textit{Stop} action and its final pose is within $d_s = 1$ m in position and within $\alpha_s = 35^\circ$ in heading relative to the target observation pose.

We evaluate navigation using Success Rate (SR), Success weighted by Path Length (SPL), Collision Rate (CR), and Inference Time(ms). A collision is recorded whenever the simulator reports contact, and CR is computed as the fraction of episodes with at least one collision.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% B Model training

\subsection{Model training}

\subsubsection{Datasets}
We utilize a diverse collection of indoor environments for training and evaluation, including the Gibson[] and Matterport3D (MP3D)[] simulation datasets. During data collection, we build a NavMesh from the scene geometry and project it onto a 2D traversability grid. To reserve a safety buffer, we inflate obstacle regions on the grid by the robot radius plus a fixed safety margin. We then run Hybrid A* on this 2D grid to generate smooth, collision-free expert trajectories that satisfy differential-drive kinematic constraints.
Each expert trajectory is represented as
\begin{equation}
\tau^{*} = \big[(x_{0}, y_{0}), (x_{1}, y_{1}), \ldots, (x_{k}, y_{k})\big],
\end{equation}
and the planned trajectories are temporally aligned with synchronized RGB-D observations, resulting in a trajectory dataset that pairs depth image with RGB image. We use the RGB image at the terminal step of each trajectory as the episode's goal image. This dataset serves as a dedicated source exclusively for training generative navigation policies.

Beyond Gibson[] and MP3D[], we incorporate 20 scenes from GO Stanford[] to further diversify the training data and reduce the sim-to
real gap. As the GO Stanford[] dataset lacks native depth information, we employ Depth Anything V2[] to generate high-fidelity depth maps. This ensures a consistent RGB-D observation space.


\subsubsection{Imitation Learning}
We pre-train the model with imitation learning using the AdamW optimizer, a learning rate of $1\times 10^{-5}$
, a batch size of 128, and 30 training epochs. Training is conducted on an NVIDIA RTX 6000 Ada GPU and typically converges within approximately 20 hours.

\subsubsection{Reinforcement Learning}
We finetune the pre-train policy in Habitat. Exploration noise is injected with standard deviations in the range of 0.08 to 0.14. Training is performed with a single parallel environment and a maximum episode length of 150 steps. We use PPO with a discount factor of 0.99, a GAE parameter of 0.95, a batch size of 1000, and an entropy regularization coefficient of 0.03. The reward function includes a terminal success reward of 5, a per-step slack penalty of -0.01, a distance-progress term defined as the change in goal distance between consecutive steps, and a collision penalty of -0.1. All RL experiments are conducted on an NVIDIA RTX 6000 Ada GPU and typically converge within approximately 30 hours.

As shown in Fig.~\ref{fig:reward_success}, the reward during training exhibits a steadily increasing trend, indicating that our reinforcement-learning fine-tuning improves the policy performance to a certain extent.

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%reward图

\begin{figure}[!t]
  \centering
  \includegraphics[width=\columnwidth]{image/reward_final.png}
  \caption{Reward curve during training.The steady rise during the RL stage demonstrates effective policy alignment with task objectives.}
  \label{fig:reward_success}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%大表

\begin{table*}[!t]
\caption{Comparison between RoamFlow and baselines on Gibson and MP3D. All methods are trained on the Gibson training split. Results on the unseen Gibson test scenes reflect in-domain performance, whereas MP3D evaluates cross-domain generalization without finetune.}
\label{tab:baseline_comparison}
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccc|cccc}
\hline
Method & Depth & Trajectory & \multicolumn{4}{c|}{Gibson} & \multicolumn{4}{c}{MP3D} \\
\cline{4-11}
 &  &  & SR(\%)$\uparrow$ & SPL(\%)$\uparrow$ & CR(\%)$\downarrow$ & Time(ms)$\downarrow$ & SR(\%)$\uparrow$ & SPL(\%)$\uparrow$ & CR(\%)$\downarrow$ & Time(ms)$\downarrow$ \\
\hline
NoMaD [] & No & Random & 43.1 & 29.4 & 17.3 & 49.1 & 34.8 & 19.7 & 25.1 & 49.4 \\
NoMaD + Distillation. [] & No & Random & 38.4 & 25.3 & 21.3 & 28.1 & 30.4 & 13.5 & 27.8 & 29.1 \\
FlowNav [] & Yes & Random & 54.7 & 34.1 & 16.1 & 47.7 & 35.1 & 24.1 & 20.3 & 46.1 \\
FlowNav + Distillation. [] & Yes & Random & 47.5 & 29.7 & 20.1 & 21.2 & 30.2 & 19.2 & 24.3 & 20.2 \\
NaviDiffusor [] & Yes & Cost-Guided & 51.1 & 45.4 & 11.8 & 89.5 & 46.1 & 34.6 & 13.3 & 90.1 \\
Navibridger [] & No & N/A & 55.4 & 37.6 & 15.8 & 46.3 & 40.8 & 23.3 & 20.5 & 43.3\\
NavDp [] & Yes & Critic-Guided & 59.3 & 47.5 & 11.6 & 61.1 & 48.1 & 34.1 & 17.5 & 62.5 \\
\hline
\textbf{RoamFlow (Ours)} & \textbf{Yes} & \textbf{Critic-Guided} & \textbf{68.7} & \textbf{61.9} & \textbf{10.9} & \textbf{19.6} & \textbf{56.1} & \textbf{47.1} & \textbf{12.2} & \textbf{19.1} \\
\hline
\end{tabular}%
}
\end{table*}


%大表
%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% C、baseline




\subsection{Baseline}


\subsubsection{Generative Navigation Baselines}
Diffusion-based navigation policies (NoMaD[], NaviDiffusor[], and NavDP[]) typically rely on iterative diffusion sampling to generate action or trajectory sequences, which can model multimodal behaviors but often incurs substantial inference overhead.
To improve efficiency, FlowNav[] replaces diffusion sampling with Conditional Flow Matching, achieving comparable performance with fewer inference steps and inference time.
NaviBridger[] starts from informative prior actions and uses a diffusion bridge to progressively align the source distribution to the target action distribution, reducing redundant multi-step denoising and yielding a better efficiency-performance trade-off.

\subsubsection{Distilled Generative Policies}

We explicitly include two distilled baselines. For diffusion distillation, we adopt a progressive distillation scheme [Karras et al. (2022)], compressing a teacher diffusion policy with multi-step denoising into a student that performs fewer (potentially one-step) updates, thereby reducing the sampling budget while retaining comparable behavior. 
For flow-matching, we leverage Rectified Flow[] to linearize the curved inference trajectories of the original model through the Reflow procedure. This trajectory-straightening technique enables an efficient 1-step distillation that significantly reduces NFE while preserving action fidelity.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% D、result

\subsection{Result}

Fig.~\ref{fig:simulation_test} illustrates representative simulation rollouts. Our policy proposes multiple candidate trajectories at each step and executes the safest, goal-directed option, yielding smooth and collision-free navigation in cluttered scenes.



%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%仿真测试图
\begin{figure}[!t]
  \centering
  \includegraphics[width=\columnwidth]{image/simulation_test.png}
  \caption{Navigation examples in simulation. At each step, our policy generates several candidate trajectories and selects one to execute (highlighted in blue). The selected trajectory is consistently safe and goal-directed.}
  \label{fig:simulation_test}
\end{figure}

\subsubsection{Baseline Comparison}

To ensure a fair comparison, we evaluate the proposed method and baselines under a unified experimental protocol. All models are trained on the same dataset split and tested in identical environments. During evaluation, identical goal image and pre-built topological graph are provided to all methods. Notably, the originally mapless baselines(NavDP[] and NaviBridger[]), are adapted to function as local planners within topological framework.


From Table~\ref{tab:baseline_comparison}, we can see that RoamFlow achieves a highest performance on the Gibson validation split. Compared with the strongest generative baseline, NavDP, it increases SR by 9.4 and SPL by 14.4, while reducing CR from 11.6 to 10.9 and reducing inference time from 61.1ms to 19.6ms. These results demonstrate that RoamFlow improves both navigation navigation quality, efficiency and safety.




\subsubsection{Ablation Study}
Our ablation study focuses on three factors: whether imitation learning (IL) pretraining is applied, whether reinforcement learning (RL) fine-tuning is performed, and whether a trajectory evaluator is used to select candidate trajectories.

\paragraph{Effect of IL Stage}
As shown in Table~\ref{tab:ablation_gibson_mp3d}, initializing the policy with IL pre-training leads to substantial performance improvements compared to training from scratch. In visual navigation, IL pre-training provides a robust behavioral prior that bootstraps early learning. Compared to training from scratch—which requires inefficient trial-and-error to learn obstacle avoidance in cluttered scenes—incorporating an IL stage significantly improves exploration efficiency and stabilizes the optimization process.

\paragraph{Effect of RL Stage}
As shown in Table~\ref{tab:ablation_gibson_mp3d}, starting from the same IL initialization, RL fine-tuning yields consistent improvements across both datasets, achieving higher SR and SPL while significantly reducing CR compared to the IL-only variant. These results indicate that RL effectively complements imitation by refining the policy through task-oriented rewards, which enhances robustness and safety via direct environment interaction in cluttered indoor scenes. Consequently, the RL stage serves as an objective-alignment step that bridges the gap between the IL prior and practical deployment requirements, further optimizing the policy toward target evaluation metrics.


\paragraph{Effect of Trajectory Evaluator}
As summarized in Table~\ref{tab:ablation_gibson_mp3d}, introducing the evaluator does not change the underlying policy, but re-ranks a set of candidate rollouts and executes the one with lower estimated risk. Compared to random selection, this simple selection mechanism consistently reduces the Collision Rate (CR), indicating improved safety in visually cluttered indoor scenes. Meanwhile, by avoiding collision-induced failures and getting stuck less often, the agent achieves a modest improvement (or a more stable retention) in Success Rate (SR) and SPL. Overall, the Trajectory Evaluator acts as a lightweight safety filter that improves trajectory reliability with minimal additional overhead, making the system more suitable for deployment.






%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%消融表

\begin{table}[!t]
\caption{Ablation analysis of the proposed components—pre-training, RL fine-tuning, and the trajectory selector—on the Gibson and MP3D validation splits.}
\label{tab:ablation_gibson_mp3d}
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{lcccccc}
\hline
Method & \multicolumn{3}{c}{Gibson} & \multicolumn{3}{c}{MP3D} \\
\cline{2-7}
 & SR$\uparrow$ & SPL$\uparrow$ & CR$\downarrow$ & SR$\uparrow$ & SPL$\uparrow$ & CR$\downarrow$ \\
\hline
\emph{Effect of IL Stage} \\
w/o IL Stage & 13.2 & 11.2 & 61.3 & 11.2 & 9.8 & 68.7 \\
\emph{Effect of RL Stage} \\
w/o RL Stage & 51.3 & 47.5 & 25.9 & 46.8 & 43.5 & 30.6 \\

\emph{Effect of Trajectory Evaluator} \\
Random Selection & 60.7 & 50.2 & 17.5 & 53.2 & 40.6 & 24.4 \\

\hline
\textbf{Full RoamFlow (Ours)} & \textbf{68.7} & \textbf{61.9} & \textbf{10.9} & \textbf{56.1} & \textbf{47.1} & \textbf{12.2} \\
\hline
\end{tabular}
\end{table}










%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%真机部署图


\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{image/deployment_2.png}
  \caption{Deployment setup.}
  \label{fig:deployment2}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% E、Physical Experiments 真机实验

\subsection{Physical Experiments}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%真机实验表
\begin{table}[!t]
  \caption{performance in physical experiments (success rate, collisions and inference time(ms)).}
  \label{tab:physical_experiments}
  \centering
  \small
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{l|ccc}
    \hline
    Method & SR$\uparrow$ & Coll./run$\downarrow$ & Time$\downarrow$ \\
    \hline

    NoMaD with Depth & 0.75 & 0.50 & 75.1 \\
    NoMaD(Distillation) with Depth& 0.70 & 0.70 & 50.2 \\
    FlowNav & 0.90 & 0.25 & 70.5\\
    FlowNav(Distillation)& 0.80 & 0.35 & 40.6 \\
    \hline
    \textbf{RoamFlow (ours)} & \textbf{1.00} & \textbf{0.10} & \textbf{32.2} \\
    \hline


    \hline
\end{tabular}
\end{table}


For real-robot experiments, our policy are deployed on a Unitree Go2 quadruped equipped with an NVIDIA Jetson Orin NX (16GB). We use ROS1 Noetic for data acquisition, and low-level motion command execution. We use an Intel RealSense D435i and stream synchronized color image and depth images as inputs to the policy.


We evaluated the models across three distinct scenarios under the goal-directed navigation task. For each scenario, we conducted 20 independent trials to ensure statistical significance. We recorded the Success Rate, the average number of collisions per episode, and the mean inference time as the primary performance metrics.


Table~\ref{tab:physical_experiments} reports success rate, collisions per run, and inference time. RoamFlow attains a higher success rate with fewer collisions at lower inference time.

Fig.~\ref{fig:deployment2} illustrates our policy's trajectory predictions during execution. As shown, the predicted trajectories consistently avoid hazardous regions, and the trajectory evaluator selects the safest candidate for execution at each decision step.

During real-robot deployment, the end-to-end inference-and-control loop is executed on-board at a frequency of 10 Hz. The inference latency consistently remains below 100 ms. Despite minor jitter in control timing, the system maintains a stable update rate, satisfying the real-time constraints required for autonomous navigation.



\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}


